Does Bidirectional Traffic Do More Harm Than Good in LoRaWAN Based LPWA Networks?

The need for low power, long range and low cost connectivity to meet the requirements of IoT applications has led to the emergence of Low Power Wide Area (LPWA) networking technologies. The promise of these technologies to wirelessly connect massive numbers of geographically dispersed devices at a low cost continues to attract a great deal of attention in the academic and commercial communities. Several rollouts are already underway even though the performance of these technologies is yet to be fully understood. In light of these developments, tools to carry out `what-if analyses' and pre-deployment studies are needed to understand the implications of choices that are made at design time. While there are several promising technologies in the LPWA space, this paper specifically focuses on the LoRa/LoRaWAN technology. In particular, we present LoRaWANSim, a simulator which extends the LoRaSim tool to add support for the LoRaWAN MAC protocol, which employs bidirectional communication. This is a salient feature not available in any other LoRa simulator. Subsequently, we provide vital insights into the performance of LoRaWAN based networks through extensive simulations. In particular, we show that the achievable network capacity reported in earlier studies is quite optimistic. The introduction of downlink traffic can have a significant impact on the uplink throughput. The number of transmit attempts recommended in the LoRaWAN specification may not always be the best choice. We also highlight the energy consumption versus reliability trade-offs associated with the choice of number of retransmission attempts.

==> LoRaSim Scalability Downlink/macros.tex <==
\newboolean{authnotes}
\setboolean{authnotes}{false}
%\setboolean{authnotes}{true}

%\newcommand{\camera}[1]{{\color{blue} #1}}
\newcommand{\camera}[1]{{#1}}

%\newcommand{\notes}[1]{{\color{red} #1}}


\ifthenelse{\boolean{authnotes}}
% if the boolean authnotes is true define the macros AND print a diagonal
% draft watermark, to remember they are in
{
\newcommand{\usman}[1]{\footnote{{\bf Usman: #1}}}
\newcommand{\parag}[1]{\footnote{{\bf Parag: #1}}}
\newcommand{\alex}[1]{\footnote{{\bf Alex: #1}}}
%\usepackage{draftwatermark}
%\SetWatermarkLightness{0.85}
%\SetWatermarkScale{1}
\newcommand{\memo}[1]{{\color{red} #1}}
%\newcommand{\usman}[1]{}
%\newcommand{\parag}[1]{}
\usepackage{draftwatermark}
\SetWatermarkText{}
%\linenumbers
}
% otherwise, just define the macros to avoid compilation errors, but ignore
% the content of the notes 
{
\newcommand{\usman}[1]{}
\newcommand{\parag}[1]{}
\newcommand{\alex}[1]{}
\usepackage{draftwatermark}
\SetWatermarkText{}
\newcommand{\memo}[1]{#1}
}

\newcommand{\fakeparagraph}[1]{\vspace{1mm}\noindent\textbf{#1}}
\newcommand{\finding}[2]{\vspace{2mm}\noindent \textbf{Finding \##1: #2\vspace{2mm}}}


\newcommand{\cmark}{\ \includegraphics[width=0.2cm]{img/tick.png}}%
\newcommand{\xmark}{ \includegraphics[width=0.2cm]{img/cross.png}}%

\newcommand{\lora}{LoRa\xspace}
\newcommand{\lorawan}{{LoRaWAN}\xspace}
\newcommand{\sigfox}{\textsc{SigFox}\xspace}
\newcommand{\ingenu}{\textsc{Ingenu}\xspace}
\newcommand{\rpma}{\textsc{RPMA}\xspace}
\newcommand{\weightless}{\textsc{Weightless}\xspace}
\newcommand{\qowisio}{\textsc{Qowisio}\xspace}
\newcommand{\dash}{\textsc{Dash7}\xspace}
\newcommand{\telensa}{\textsc{Telensa}\xspace}
\newcommand{\nbiot}{\textsc{NB-I}o\textsc{T}\xspace}
\newcommand{\nwave}{\textsc{Nwave}\xspace}
\newcommand{\catzero}{\textsc{LTE-Cat0}\xspace}
\newcommand{\catm}{\textsc{LTE-M}\xspace}

\newcommand{\aloha}{\textsc{Aloha}\xspace}

\newcommand{\lorawantm}{\textsc{LoR}aWAN\texttrademark\xspace} 

\newcommand{\loraalliance}{\textsc{LoR}a\texttrademark\xspace Alliance\xspace} 

\newcommand{\ul}{\textsc{(ul)}\xspace}
\newcommand{\dl}{\textsc{(dl)}\xspace}

\newcommand{\urban}{\textsc{(urban)}\xspace}
\newcommand{\rural}{\textsc{(rural)}\xspace}

\newcommand{\ism}{\textsc{ISM}\xspace}

\newcommand{\subghz}{\textsc{Sub-GHz}\xspace}


\newcommand{\wrt}{w.r.t.\ }
\newcommand{\nd}{\textsc{ND}\xspace}

